Probing Kilonova Ejecta Properties Using a Catalog of Short Gamma-Ray Burst Observations

The discovery of GW170817 and GRB 170817A in tandem with AT 2017gfo cemented the connection between neutron star mergers, short gamma-ray bursts (GRBs), and kilonovae. To investigate short GRB observations in the context of diverse kilonova behavior, we present a comprehensive optical and near-infrared (NIR) catalog of 85 bursts discovered over 2005-2020 on timescales of $\lesssim12$ days. The sample includes previously unpublished observations of 23 bursts, and encompasses both detections and deep upper limits. We identify 11.8% and 15.3% of short GRBs in our catalog with upper limits that probe luminosities lower than those of AT 2017gfo and a fiducial NSBH kilonovae model (for pole-on orientations), respectively. We quantify the ejecta masses allowed by the deepest limits in our catalog, constraining blue and `extremely blue' kilonova components of 14.1% of bursts to $M_{\rm ej}\lesssim0.01-0.1 M_{\odot}$. The sample of short GRBs is not particularly constraining for red kilonova components. Motivated by the large catalog as well as model predictions of diverse kilonova behavior, we investigate modified search strategies for future follow-up to short GRBs. We find that ground-based optical and NIR observations on timescales of $\gtrsim 2$ days can play a significant role in constraining more diverse outcomes. We expect future short GRB follow up efforts, such as from the {\it James Webb Space Telescope}, to expand the reach of kilonova detectability to redshifts of $z\approx 1$.

==> abs_talk.tex <==
Summer AAS:

Probing Kilonova Ejecta Properties Using a Catalog of Short Gamma-Ray Burst Observations

The discovery of GW170817 and GRB170817A in tandem with AT2017gfo cemented the connection between neutron star mergers, short gamma-ray bursts (GRBs), and kilonovae. While gravitational wave detectors are on hiatus, short GRBs present an exciting avenue for continued kilonova searches. In this talk, I will present our comprehensive catalog of optical and near-infrared observations of 85 short GRBs discovered in the last 15 years, including detections of kilonova candidates, low-luminosity afterglows, and deep upper limits. I will discuss how this catalog reveals diversity in kilonovae uniformly observed from a pole-on viewing angle, including that deep upper limits of a number of bursts probe lower luminosities than AT2017gfo. In addition, I will show that past observational follow-up of short GRBs is more constraining of lanthanide-poor rather than lanthanide-rich kilonovae. Future targeted follow-up of short GRBs may uncover further kilonovae diversity and provide insights to the progenitors and remnant of a burst.


For EAS BH-NS conference:

The discovery of GW170817 and GRB170817A in tandem with AT2017gfo cemented the connection between neutron star mergers, short gamma-ray bursts (GRBs), and kilonovae. Though not yet confirmed, BH-NS mergers are a second suspected progenitor of short GRBs. The kilonova ejecta of BH-NS mergers is expected to be more rich in lanthanide elements than that of NS-NS mergers, a distinct electromagnetic signature that may provide clues to a short GRB's progenitor. In this talk, I will present our comprehensive catalog of optical and near-infrared observations of 85 short GRBs discovered in the last 15 years, including detections of kilonova candidates, low-luminosity afterglows, and deep upper limits. I will discuss how this catalog reveals diversity in kilonovae uniformly observed from a pole-on viewing angle through comparisons to models for various progenitors and remnants, including that of a BH-NS system. In addition, I will show that past observational follow-up of short GRBs is more constraining of lanthanide-poor rather than lanthanide-rich kilonovae. Future targeted follow-up of short GRBs may uncover further kilonovae diversity and provide observational clues to the progenitors and remnant of a burst.

==> published.tex <==
\startlongtable
\tabletypesize{\footnotesize}
\begin{deluxetable*}{lclrCRrRc}
\centering
\tablecolumns{9}
\tabcolsep0.07in
\tablewidth{0pc}
\tablecaption{Log of Published Sample of Short GRB Observations
\label{tab:pub}}
\tablehead {
\colhead {GRB}		&
\colhead {$z$}		&
\colhead {Telescope/Instrument}	&
\colhead {$\delta t$}	&
\colhead {Filter}	&
\colhead {Detection/Limit}	&
\colhead {Error}	&
\colhead {$\nu L_{\nu}$}	&
\colhead {Reference}	
\\
\colhead {}		&
\colhead {}		&
\colhead {}	&
\colhead {(days)}	&
\colhead {}        &
\colhead {(AB mag)}	&
\colhead {(AB mag)}	&
\colhead {(erg/s)}	&
\colhead {}		
}
\startdata
050509B & 0.225 & 6.0BTA/SCORPIO & 2.67 & R & $>$26.0 &   & < 1.1 \times 10^{41} & 1 \\
 &  & WIYN/OPTIC & 0.09 & r & $>$24.2 &   & < 5.5 \times 10^{41} & 2 \\
 &  & WIYN/OPTIC & 0.10 & r & $>$23.8 &   & < 7.8 \times 10^{41} & 2 \\
 &  & WIYN/OPTIC & 0.10 & r & $>$23.9 &   & < 7.7 \times 10^{41} & 2 \\
 &  & WIYN/OPTIC & 0.11 & r & $>$24.1 &   & < 6.1 \times 10^{41} & 2 \\
 &  & Keck-I/LRIS & 1.08 & R & $>$25.6 &   & < 1.5 \times 10^{41} & 3 \\
 &  & VLT/FORS & 1.85 & R & $>$25.1 &   & < 2.4 \times 10^{41} & 4 \\
050709$^{\ddagger}$ & 0.161 & Danish tel./DFOSC & 1.41 & R & 23.0 & 0.1 & 8.1 \times 10^{41} & 5 \\
 &  & VLT/FORS2 & 2.47 & R & 24.0 & 0.1 & 3.2 \times 10^{41} & 6 \\
 &  & Danish tel./DFOSC & 2.50 & R & 23.7 & 0.2 & 4.1 \times 10^{41} & 5 \\
 &  & VLT/FORS1 & 4.36 & V & $>$25.0 & & < 1.6 \times 10^{41} & 6 \\
 &  & $HST$/ACS & 5.60 & F814W & 25.1 & 0.1 & 1.2 \times 10^{41}& 7 \\
 &  & $HST$/ACS & 9.80 & F814W & 25.8 & 0.1 & 6.0 \times 10^{41} & 7 \\
050724A & 0.257 & Magellan/Baade/PANIC & 1.45 & K & $>$22.1 & & < 1.5 \times 10^{42}  &  9 \\
 &  & VLT/FORS1 & 1.45 & I & 22.8 & 0.1 & 2.2 \times 10^{42} & 8 \\
 &  & Swope 40 in. & 1.53 & I & $>$21.5 &  & < 7.0 \times 10^{41} & 9 \\
 &  & VLT/FORS1 & 1.46 & R & 22.6 & 0.1 & 3.3 \times 10^{42} & 8 \\
 &  & VLT/FORS1 & 3.46 & I & 25.1 & 0.3 & 2.5 \times 10^{41} &  8 \\
050813 & 0.72 & CAHA/CAFOS & 0.55 & I & $>$23.2 &  & < 1.6 \times 10^{43} & 10 \\
 & & CAHA/CAFOS & 0.59 & R & $>$23.5 &  & < 1.6 \times 10^{43} & 10 \\
050906$^{a}$ & 0.5$^{\dagger}$ & VLT/FORS2 & 0.89 & R & $>$26.0 &  & < 7.1 \times 10^{41} & 11 \\
051210 & 0.5$^{\dagger}$ & Magellan/Clay/LDSS3 & 0.81 & r & $>$25.9 &  & 9.3 \times 10^{42} &  12  \\
051221A & 0.546 & Gemini-N/GMOS & 6.16 & r & $>$24.6 &  & < 3.0 \times 10^{42} & 13 \\
060121 & 0.5$^{\dagger}$ & WIYN & 1.40 & R & 24.9 & 0.2 & 1.9 \times 10^{42} & 14 \\
060313 & 0.5$^{\dagger}$ & Gemini-S/GMOS & 10.0 & r & $>$24.7 &  & < 2.2 \times 10^{42} &  12  \\
060502B & 0.287 & Gemini-N/GMOS & 0.70 & R & $>$24.3 &  & < 8.9 \times 10^{41} & 15 \\
060614$^{\ddagger}$ & 0.125 & VLT/FORS1 & 3.86 & I & 24.2 & 0.6 & 1.3 \times 10^{41} & 16 \\
 & & VLT/FORS1 & 3.87 & R & 25.5 &  0.3 & 4.6 \times 10^{40} & 16 \\
 & & VLT/FORS1 & 4.85 & R & 25.1 & 0.3  & 6.6 \times 10^{40} & 16 \\
 & & VLT/FORS1 & 6.74 & R & 25.5 &  0.3 &  4.6 \times 10^{40} & 16 \\
 & & VLT/FORS1 & 7.84 & I & 25.1 & 0.4  &  5.7 \times 10^{40} & 16 \\
061201 & 0.111 & VLT/FORS2 & 0.36 & I & 22.8 & 0.1 & 3.6 \times 10^{41} & 17 \\
 & & VLT/FORS2 & 0.38 & R & 23.2 & 0.1 & 3.0 \times 10^{41} & 17 \\
 & & VLT/FORS2 & 1.38 & I & $>$24.0 &  & < 1.2 \times 10^{41}  & 17 \\
 & & VLT/FORS2 & 3.39 & I & $>$24.4 &  & < 8.0 \times 10^{40}  & 17  \\
061217$^{a}$ & 0.827 & Magellan/Clay/LDSS3 & 0.12 & r & $>$23.1 &  & < 3.2 \times 10^{42} &  12  \\
070406$^{a}$ & 0.5$^{\dagger}$ & NOT/ALFSOC & 1.02 & R & $>$23.6 &  & < 5.9 \times 10^{42} & 18 \\
070429B & 0.902 & Gemini-S/GMOS & 0.20 & R & $>$24.7 &  & < 9.8 \times 10^{42} & 19 \\
 & & Blanco/ISPI & 1.13 & J & $>$22.4 &  & < 4.0 \times 10^{43} & 20 \\
070707 & 0.5$^{\dagger}$ & VLT/ISAAC & 2.54 & J & $>$24.5 &  & < 1.4 \times 10^{42} & 21 \\
070714B & 0.923 & TNG/NICS & 1.00 & J & $>$21.5 &  & < 9.3 \times 10^{43} & 22 \\
070724A & 0.457 & Gemini-N/GMOS & 0.10 & g & $>$23.5 &  & < 7.0 \times 10^{42} & 23 \\
070729 & 0.8 & ESO/MPG/GROND & 0.35 & R & $>$24.7 &  & < 7.0  \times 10^{42} & 24 \\
 &  & ESO/MPG/GROND & 0.35 & J & $>$22.7 &  & < 2.3 \times 10^{43} & 24 \\
070809 & 0.473 & Keck-I/LRIS & 0.47 & g & 25.1 & 0.2 & 1.8 \times 10^{42}  & 25 \\
 & & Keck-I/LRIS & 0.47 & R & 23.9 & 0.3 & 4.2 \times 10^{42} & 25 \\
  & & Keck-I/LRIS & 1.46 & g & $>$25.4 &  & < 1.4 \times 10^{42}  & 25 \\
 & & Keck-I/LRIS & 1.46 & R & 24.8 & 0.3 & 1.8 \times 10^{42} & 25 \\
071112B$^{a}$ & 0.5$^{\dagger}$ & Magellan/Clay/LDSS3 & 0.26 & r & $>$23.1 &  & < 9.3 \times 10^{42} & 26 \\
 & & ESO/MPG/GROND & 0.40 & J & $>$21.6 &  & < 2.0 \times 10^{42} & 24 \\
080503 & 0.5$^{\dagger}$ & Gemini-N/GMOS & 0.04 & r & $>$25.6 & & < 9.7 \times 10^{41} & 27 \\
 & & Gemini-N/GMOS & 0.05 & g & 26.5 & 0.2 & 5.5 \times 10^{41} & 27 \\
 & & Keck-I/LRIS & 0.05 & R & $>$25.6 &   & < 9.9 \times 10^{41} &   27 \\
 & & Gemini-N/GMOS& 0.06 & r & $>$26.6 &   & < 3.8 \times 10^{41} &  27 \\
 & & Gemini-N/GMOS & 0.08 & i & $>$26.7 &   & < 3.0 \times 10^{41} &  27 \\ 
 & & Gemini-N/GMOS & 0.09 & z & $>$25.9 &   &  < 5.2 \times 10^{41} &  27 \\
 & & Gemini-N/GMOS & 1.08 & r & 25.3 & 0.1 & 1.3 \times 10^{42} &  27  \\
 & & Gemini-N/GMOS & 1.98 & r & 25.5 & 0.2 &  1.1 \times 10^{42} &  27 \\
 & & Gemini-N/GMOS & 2.09 & g & 26.3 & 0.3 & 7.1 \times 10^{41} &  27  \\
  & & Gemini-N/GMOS & 3.08 & r & 25.7 & 0.3 &  1.1 \times 10^{42} &  27 \\
 & & Gemini-N/GMOS & 4.05 & r & 26.1 & 0.2 & 7.1 \times 10^{41} &  27  \\
 & & $HST$/WFPC2 & 5.36 & F606W & 26.9 &  0.2 &  3.0 \times 10^{41} & 27 \\
080905A & 0.122 & NOT/ALFSOC & 0.35 & R & 24.3 & 0.5 & 1.4 \times 10^{41} & 28 \\
 & & VLT/FORS2 & 0.60 & R & 24.5 & 0.3 & 1.1 \times 10^{41} & 28 \\
 & & ESO/MPG/GROND & 0.73 & g & $>$22.5 &   & < 8.7 \times 10^{41} & 24 \\
 & & VLT/FORS & 1.50 & R & $>$25.2 &   & < 5.7 \times 10^{40} & 28 \\
090305$^{a}$ & 0.5$^{\dagger}$ & Gemini-S/GMOS & 0.90 & r & $>$25.7 &   & < 3.7 \times 10^{40} & 29 \\
090515 & 0.403 & Gemini-N/GMOS  & 0.07 & r & 26.3 & 0.1 & 3.1 \times 10^{41} & 17 \\
 & & Gemini-N/GMOS & 1.04 & r & 26.5 & 0.3 & 2.6 \times 10^{41} & 29 \\
090621B & 0.5$^{\dagger}$ & RTT150/TFOSC & 0.03 & r & $>$23.2 &  & < 8.9 \times 10^{42} & 30 \\
091109B & 0.5$^{\dagger}$ & VLT/FORS2 & 0.25 & R & 24.3 & 0.1 & 3.2 \times 10^{42} & 29 \\
 &  & VLT/HAWK-I & 0.30 & K & $>$24.1 &  & < 1.1 \times 10^{42} & 29 \\
 &  & VLT/HAWK-I & 0.35 & J & $>$22.9 &  & < 5.7 \times 10^{42} & 29 \\
 & & VLT/FORS2 & 0.43 & R & 24.6 & 0.2 & 2.4 \times 10^{42} & 29  \\
 & & VLT/FORS2 & 1.32 & R & $>$25.8 &   & < 8.0 \times 10^{41} & 29  \\
100206 & 0.407 & ESO/MPG/GROND & 0.49 & i & $>$23.3 &  & < 4.0 \times 10^{42} & 24 \\
 &  & Gemini-N/GMOS & 0.65 & i & $>$25.8 &   & < 4.3 \times 10^{41} & 31 \\
100625A & 0.452 & ESO/MPG/GROND & 0.51 & g & $>$23.6 &  & < 6.0 \times 10^{42} & 24 \\
 &  & Magellan/PANIC & 1.41 & J & $>$23.9 &   & < 1.9 \times 10^{42} & 24 \\
100628A & 0.5$^{\dagger}$ & Gemini-N/GMOS & 0.05 & i & $>$24.1 &  & < 3.9 \times 10^{42} & 32 \\
 &  & Magellan/PANIC & 0.74 & J & $>$22.1 &  & < 1.3 \times 10^{43} & 32 \\
100702A & 0.5$^{\dagger}$ & ESO/MPG/GROND & 0.07 & r' & $>$23.2 &  & < 9.1 \times 10^{42} & 24 \\
101219A & 0.718 & Gemini-S/GMOS & 0.04 & i & $>$24.9 &   & < 3.5 \times 10^{42}& 33 \\
 &  & Magellan/FourStar & 0.05 & J & $>$23.6 &   & < 7.9 \times 10^{42} & 33 \\
110420B$^{a}$ & 0.5$^{\dagger}$ & Magellan/IMACS & 0.44 & r & $>$23.5 &   & < 6.5 \times 10^{42} & 32 \\
111020A & 0.5$^{\dagger}$ & Gemini-S/GMOS & 0.74 & i & $>$24.4 &  & < 2.4 \times 10^{42} & 34 \\
 & & VLT/HAWK-I & 0.77 & J & $>$24.5 & & < 2.4 \times 10^{42}  & 29 \\
111117A & 2.211 & GTC/OSIRIS & 0.34 & r & $>$24.9 &   & < 7.1 \times 10^{43} & 35 \\
 &  & Gemini-S/GMOS & 0.57 & r & $>$25.5 &   & < 4.1 \times 10^{43} & 36 \\
120521A & 0.5$^{\dagger}$ & ESO/MPG/GROND & 0.78 & r & $>$24.0 &   & < 4.1 \times 10^{42} & 37 \\
120817B & 0.5$^{\dagger}$ & LCO/duPont/WFCCD & 1.00 & R & $>$23.5 &   & < 7.0 \times 10^{42} & 38 \\
130515A & 0.5$^{\dagger}$ & Gemini-S/GMOS & 0.03 & r & $>$23.5 &   & < 6.5 \times 10^{42} & 39 \\
130603B$^{\ddagger}$ & 0.356 & $HST$/ACS & 9.37 & F606W & $>$27.7 &  & < 7.7 \times 10^{40} & 40,41 \\
 & & $HST$/WFC3 & 9.49 & F160W & 25.8 & 0.2  &  1.4 \times 10^{41} & 40,41 \\
130716A & 0.5$^{\dagger}$ & Gemini-N/GMOS & 0.81 & r & $>$25.0 &  & < 9.7 \times 10^{41} & 32 \\
131004A & 0.717 & HJT/RATIR & 0.30 & r & $>$23.4 &  & < 1.7 \times 10^{43} & 42 \\
 &   & HJT/RATIR & 0.30 & i & $>$23.2 &  & < 1.7 \times 10^{43} & 42 \\
 &   & HJT/RATIR & 0.30 & Z & $>$22.7 &  & < 2.3 \times 10^{43} & 42 \\
 &   & HJT/RATIR & 0.30 & Y & $>$22.2 &  & < 3.2 \times 10^{43} & 42 \\
 &   & HJT/RATIR & 0.30 & J & $>$22.5 &  & < 2.0 \times 10^{43} & 42 \\
 &   & HJT/RATIR & 0.30 & H & $>$22.5 &  & < 1.5 \times 10^{43} & 42 \\
131224A$^{a,b}$ & 0.5$^{\dagger}$  & GTC & 1.11 & z & $>$23.1 &  & < 3.1 \times 10^{42} & 43 \\
140402A$^{a}$ & 0.5$^{\dagger}$ & Magellan/Baade/IMACS & 1.21 & r & $>$25.0 &  & < 1.7 \times 10^{42} & 32 \\
140516 & 0.5$^{\dagger}$ & NOT/ALFSOC & 0.08 & R & $>$24.7 &  & < 2.3 \times 10^{42} & 44 \\
 &  & Subaru/IRCS+AO188 & 0.48 & K' & $>$24.1 &  & < 1.1 \times 10^{42} & 45 \\
 &  & Gemini-N/GMOS & 0.52 & i & $>$26.1 &  & < 5.2 \times 10^{41} & 32 \\
 &  & HJT/RATIR & 0.54 & J & $>$22.0 &  & < 1.4 \times 10^{42} & 46 \\
140606A$^{a}$ & 0.5$^{\dagger}$ & BTA & 0.39 & V & $>$24.2 &  & < 4.5 \times 10^{42} & 43 \\
 &  & BTA & 0.43 & R_c & $>$26.0 &  & < 7.0 \times 10^{41} &  43  \\
140619B$^{a,c}$ & 0.5$^{\dagger}$ & Magellan/Baade/FourStar & 1.48 & J & $>$22.9 &  & < 6.1 \times 10^{42} & 32 \\
140622A & 0.959 & GTC & 0.78 & r & $>$25.4 &  & < 4.6 \times 10^{42} & 43 \\
140930B & 0.5$^{\dagger}$ & GTC & 3.14 & r & $>$24.5 &  & < 2.8 \times 10^{42} & 43 \\
150101B$^{\ddagger}$ & 0.134 & Magellan/Baade/IMACS & 1.66 & r & 23.0 & 0.2 & 2.4 \times 10^{42} & 47 \\
 &  & Magellan/Baade/IMACS & 2.63 & r & 23.5 & 0.3 & 5.2 \times 10^{41} & 47 \\
 &  & Gemini-S/GMOS & 10.71 & r & $>$24.2 & & < 1.4 \times 10^{43} & 47 \\
150424A & 1.0 & ESO/MPG/GROND & 1.81 & r' & 23.1 & 0.1 & 5.5 \times 10^{43} & 48 \\
 & & ESO/MPG/GROND & 1.81 & i' & 23.0 & 0.1 & 4.7 \times 10^{43} & 48 \\
 & & ESO/MPG/GROND & 1.81 & z' & 22.6 & 0.1 & 5.7 \times 10^{43} & 48 \\
  & & $HST$/WFC3 & 6.64 & F606W & 25.9 & 0.1 & 4.1 \times 10^{42} & 49 \\
 & & $HST$/WFC3 & 6.68 & F125W & 25.3 & 0.1 & 3.7 \times 10^{42} & 49 \\
 & & $HST$/WFC3& 6.71 & F160W & 25.1 & 0.1 & 3.3 \times 10^{42} & 49  \\
 & & $HST$/WFC3 & 9.23 & F606W & 26.9 & 0.1 & 1.6 \times 10^{42} & 49  \\
 & & $HST$/WFC3 & 9.26 & F125W & 26.3 & 0.2 & 1.5 \times 10^{42} & 49  \\
 & & $HST$/WFC3 & 9.30 & F160W & 25.8 & 0.1 & 1.8 \times 10^{42} & 49 \\
151228A$^{a}$ & 0.5$^{\dagger}$ & GTC & 1.14 & i & $>$23.7 &  & < 5.1 \times 10^{42} & 43 \\
160821B$^{\ddagger}$ & 0.1616 & WHT/ACAM & 1.06 & r & 23.8 & 0.1 &  3.8 \times 10^{41} &  50 \\
 & & WHT/ACAM & 1.08 & z & 23.6 & 0.2 &  3.1 \times 10^{41} & 50  \\
 & & GTC/CIRCE & 1.94 & H & $>$23.8 &   & < 1.5 \times 10^{41} & 51 \\
 & & NOT/ALFOSC & 1.95 & r & 24.8 & 0.1 &  1.5 \times 10^{41} & 50 \\
 & & GTC/CIRCE & 1.96 & J & $>$24.0 &   & < 1.7 \times 10^{41} & 51 \\
 & & NOT/ALFOSC & 1.99 & z & 23.9 & 0.2 &  2.4 \times 10^{41} & 50 \\
 & & GTC/OSIRIS & 2.02 & g & 25.6 & 0.2 &  2.5 \times 10^{41} & 50  \\
 & & GTC/OSIRIS & 2.03 & r & 24.8 & 0.1 &  1.6 \times 10^{41} &  50 \\
 & & GTC/OSIRIS  & 2.04 & i & 24.5 & 0.1 &  1.7 \times 10^{41} &  50 \\
 & & GTC/OSIRIS & 2.04 & z & 24.3 & 0.2 &   1.6 \times 10^{40} & 50 \\
 & & $HST$/WFC3/UVIS & 3.64 & F606W & 25.9 & 0.1 &  5.6 \times 10^{40} & 50  \\
 & & $HST$/WFC3/IR & 3.71 & F160W & 24.4 & 0.1 &  8.4 \times 10^{40} &  50 \\
 & & $HST$/WFC3/IR & 3.76 & F110W & 24.7 & 0.2 &  8.7 \times 10^{40} &  50 \\
 & & GTC/OSIRIS & 3.98 & g & 26.0 & 0.2 &  6.7 \times 10^{40} & 50 \\
 & & GTC/OSIRIS & 4.00 & i & 25.7 & 0.4 &  5.5 \times 10^{40} &  50 \\
 & & GTC/OSIRIS & 4.99 & r & 26.1 & 0.3 &  4.6 \times 10^{ 42} & 50  \\
 & & GTC/OSIRIS & 6.98 & g & 26.9 & 0.2 &  2.9 \times 10^{40} &  50 \\
 & & GTC/OSIRIS & 9.97 & i & $>$25.6 &   & < 6.0 \times 10^{40} &  50 \\
 & & GTC/OSIRIS & 10.00 & g & $>$25.7 &   & < 8.7 \times 10^{40} &   51 \\
 & & $HST$/WFC3/UVIS & 10.01 & F606W & $>$26.1 &   & < 4.6 \times 10^{40} & 50 \\
 & & $HST$/WFC3/UVIS & 10.40 & F606W & 27.7 & 0.1 &  1.1 \times 10^{40} &  50 \\
 & & $HST$/WFC3/IR & 10.46  & F160W & 26.6 & 0.2 &  1.2 \times 10^{40} &  50 \\
 & & $HST$/WFC3/IR & 10.53 & F110W & 26.7 & 0.2 &   1.4 \times 10^{40} & 50 \\
161104A & 0.65 & Gemini-S/GMOS & 0.72 & r & $>$25.4 &  & < 1.2 \times 10^{42} & 52 \\
180418A & 1.0$^{\dagger}$ & Gemini-N/GMOS & 4.80 & r & $>$25.2 &  & < 1.4 \times 10^{42} & 53 \\
181123B & 1.754 & Keck I/MOSFIRE & 0.43 & J & $>$23.2 &  & < 9.9 \times 10^{43} & 54 \\
 & & MMT/MMIRS & 2.27 & J & $>$23.3 &  & < 9.0 \times 10^{43} & 55 \\
200522A$^{\ddagger}$ & 0.5537 & $HST$/WFC3 & 3.52 & F125W & 24.8 & 0.1 &  1.4 \times 10^{42} &  55 \\
 & & $HST$/WFC3 & 3.66 & F160W & 24.9 & 0.1 &  9.8 \times 10^{41} & 55 \\
%  & & $HST$/WFC3 & 16.38 & F125W & $>$27.5 &  &  \\
\enddata
\tablecomments{This sample includes previously published (i) detections of kilonova candidates (marked with $\ddagger$ symbols), (ii) deep ($m \gtrsim 21.5$) upper limits, and (iii) low-luminosity ($\nu L_{\nu} \lesssim 5 \times 10^{41}$ erg s$^{-1}$) afterglow detections. \\
\textbf{References}: (1) - \cite{Castro-Tirado+05}, (2) - \cite{Bloom+06}, (3) - \cite{GCN3409}, (4) - \cite{Hjorth+05}, (5) - \cite{Hjorth+05b}, (6) - \cite{Covino+06}, (7) - \cite{Fox+05}, (8) - \cite{Malesani+07}, (9) - \cite{Berger+05}, (10) - \cite{Ferrero+07}, (11) - \cite{Levan+08}, (12) - \cite{Berger+07}, (13) - \cite{Soderberg+06},  (14) - \cite{levan+06}, (15) - \cite{Price+06}, (16) - \cite{Jin+15}, (17) - \cite{Stratta+07}, (18) - \cite{Malesani+07b}, (19) - \cite{GCN6774}, (20) - \cite{Nysewander+07}, (21) - \cite{Piranomonte+07}, (22) - \cite{Covino+07}, (23) - \cite{Berger+09}, (24) - \cite{Guelbenzu+12}, (25) - \cite{Perley+07}, (26) - \cite{BergerChallis07}, (27) - \cite{Perley09}, (28) - \cite{Rowlinson+10}, (29) - \cite{Tunnicliffe+14}, (30) - \cite{Galeev+09}, (31) - \cite{Perley+12},
(32) - \cite{fong+15}, (33) - \cite{Fong+13}, (34) - \cite{Fong+12}, (35) - \cite{Sakamoto+13}, (36) - \cite{Margutti+12}, (37) - \cite{Rossi+12}, (38) - \cite{Fong+12-GCN}, (39) - \cite{CenkoCucchiara13}, (40) -  \cite{berger+13}, (41) - \cite{Tanvir+13}, (42) - \cite{Littlejohns+13}, (43) - \cite{pandey+19}, (44) - \cite{GCN16290}, (45) - \cite{Minowa+14}, (46) - \cite{Butler+14}, (47) - \cite{Fong+16}, (48) - \cite{Knust+17}, (49) - \cite{Jin+18}, (50) - \cite{lamb+19}, (51) - \cite{troja+19}, (52) - \cite{Nugent+20}, (53) - \cite{RoucoEscorial+20}, (54) - \cite{Paterson+20}, (55) - \cite{fong+20}. \\
\textbf{Redshift References}: \cite{Bloom+06}, %050509b
\cite{Berger+05}, %050724A
\cite{Prochaska+06}, %050813
\cite{Soderberg+06}, %051221A
\cite{Bloom+07}, %060502B
\cite{GCN5275}, %060614
\cite{Stratta+07}, %061201
\cite{GCN5965}, %061217
\cite{Cenko+08}, %070429B, 070714B
\cite{Berger+09}, %070724A
\cite{Nugent+20}, %070729
\cite{Berger10}, %070809
\cite{Rowlinson+10b}, %080905A
\cite{Rowlinson+10}, %090515
\cite{Perley+12}, %100206A
\cite{Fong+13}, %100625A and 101219A
\cite{Selsing+18}, %111117A and 140622A
\cite{GCN15307}, %131004A
\cite{fong+15}, \cite{Fong+16}, \cite{Jin+18}, \cite{lamb+19}, \cite{troja+19}, \cite{Nugent+20}, \cite{RoucoEscorial+20}, \cite{Paterson+20}, \cite{fong+20}. \\
Unless noted, all bursts are detected by \textit{Swift}-BAT and \textit{Swift}-XRT. \\
$^{\dagger}$ Redshift unknown, $z=0.5$ taken as fiducial value in analysis, except for GRB\,180418A which is assumed to be $z=1.0$ (c.f., \citealt{RoucoEscorial+20}). \\
$^{\ddagger}$ Kilonova candidate \\
$^{a}$ Burst does not have an X-ray afterglow found by \textit{Swift}-XRT. \\
$^{b}$ Burst detected by \textit{INTEGRAL}-IBIS/ISGRI, not detected by \textit{Swift}-BAT. \\
$^{c}$ Burst detected by \textit{Fermi}-GBM, \textit{Fermi}-LAT and by \textit{Suzaku}-WAM, not detected by \textit{Swift}-BAT.}
\end{deluxetable*}


==> ref_report.tex <==
##### comments to editor only go here

* We thank the editor for their thoughtful point about the observations of GRB 160624A now published in O'Connor et al., 2021 and for working with us to find a resolution. We have updated our text to reflect that (i) their publication has been accepted during our referee process, and (ii) our work presents an independent analysis of these observations that results in upper limits ~0.3 magnitudes deeper, which is significant in the context of our analysis (in terms of inferred ejecta masses). Specifically, we have combined our previous "new" and "published" samples into one "total" sample table (in the Appendix). In the reference column for the GRB 160624A observations we reference both O'Connor et al., 2021 and our work, with a footnote describing the small discrepancy in derived upper limits from our separate analysis. We have also moved our description of 160624A observations from Section 2.1 to Section 2.3 (literature sample), where we also explicitly state that these observations have been published in O'Connor et al., 2021.

* By and large we have accepted the referee's suggestions and incorporated them into our work (and a genuine restructuring resulted, which we believe makes the paper punchier and better). However, we wanted to explain a few instances in which we did not accept the referee's (minor) suggestions. First, we chose not to remove any of the GRB/GW170817/AT2017gfo references in the introduction, in the spirit of fairness to the many authors who contributed to this discovery. We also chose to keep language about how the viewing angle of short GRBs may be biasing us to observe bluer kilonovae than those observed from GW searches. We read the works the referee cited and determined that they stated viewing angle cannot explain all short GRB kilonova diversity, leaving the door open that it may be one of a few contributing factors. Finally, we declined the referee's suggestion that we remove all but the last paragraph of new section 5.1 on the r-process implications of our work, as we felt that this is one of the most significant promises of kilonovae.

###


Reviewer #1:
General comment:
################

I find this manuscript worth of publication because a) expands the analysis presented in previous work, 
b) includes comparison with not one but several theoretical models, and c) new data is published. 

However, some paragraph are too long because the same concepts more than once or are even not relevant for this work. This is unfortunate, because it makes the paper too long and difficult to read. Therefore, my first general comment is to remove unnecessary text. I give several examples below in the comments. They are divided in major, normal, and minor. I refer to the lines in the referee version of the draft with, e.g., l.33 meaning line number 33.

* We are extremely appreciative of the anonymous referee for their constructive and thorough feedback on our manuscript. We have addressed the majority of comments in the manuscript, and have provided detailed explanations for the few points we decided not to include in the final draft. In particular, we have seriously considered the referee's point about unnecessary text and have consolidated information on our analysis. We have moved old Section 5.1 to Section 3.3 and old Section 5.2 to Sections 4.3/4.4, which allowed us to cut several repetitive summary statements. In addition, we have done a careful read of the text and have cut verbose, repetitive or irrelevant language. Finally, we combined former Tables 1 ("New observations") and A1 ("Published observations") into a single Table A1 ("Total Sample").

Please find responses to each specific comment below.

Major comments:
#############

- Redshifts

The authors compare the size of their sample to Gompertz+18 and Rossi+19 which however are limited only to GRBs with a measured redshift (from the putative host usually). This is unfair because in this work many GRBs have a redshift fixed to be the median of the redshift distribution. The authors should clearly state how many GRBs have a measured redshift. I appreciate that at some point (Sec.5.1, lines~975) the authors discuss the possible bias and assume also redshift z=1. But this approach should be introduced in section 2, together with the first assumption for z=0.5 and the bias should be discussed for all cases, not just for R_AT2017gfo. I believe this will make the analysis stronger.

Moreover, the authors are certainly aware of the problem with the accuracy of the redshift of short GRBs. For example, 070809, 080905A, 090515, 060121, 070809, 150424A (see below) could be chance alignment. Only in very few cases the redshift could be measured from the afterglow itself. The fact that in some of these cases, like GRB 070809, there is a claim for a KN component in the afterglow, makes the problem relevant for this work and must at least be acknowledged. 

* We thank the referee for this important point. We have made a new Section 2.1 describing overall sample characteristics, and we have added sentences in the second paragraph of Section 2 which acknowledge the possibility that chance alignment could play a role in improper host associations for some of these bursts. We have also removed language on direct comparison by numbers to other samples.

- Sample:
I find the sample not clearly presented. How many bursts have a detection and how many have a certain redshift? Given that Gompertz et al., Ascenzi et al., and Rossi et al., have limited their work to events with a redshift measurement, 
the reader would benefit of such information. 

* Thank you for this point. We have restructured the 2nd paragraph of Section 2 to more clearly present the sample. We specifically note how many bursts in our sample have known and unknown redshifts, and how many have claimed kilonova detections.

- The sample used to determine quantitative constraints on KN parameters (section 4) is not clear. How the 14 GRBs have been selected? See line 652.

* The first paragraph of Section 4.1 has been rewritten to better convey the criteria we used to choose bursts for the ejecta mass analysis

comments:
########

- Sec: 2 line>200 I feel this is not very clear. The reader would benefit if the author could be more specific on numbers: e.g., "(i) unpublished observations of 23(?) GRBs ...". If I understand correctly, the "new" sample is made by bursts of sources i) and ii). If so, please write this clearly.

* We have combined the "new" and literature samples to help clarify this issue. The section has also been rewritten for clarity to the point about redshifts above.

- l.327 GRB 070809 should be included here. See Jin et al., Nat. Astron. 4, 77-82 (2020). Moreover, Gao et al., ApJ 837, 50 (2017) found evidence of KN in GRBs 050724, 061006, and 070714B, but see Rossi et al., 2020, that considers only 050724 and 070714B. They are very luminous and Gao claims they are powered by a magnetar, perhaps similar to 200522A? Moreover, although 080503 has no secure redshift, there is a claim and it should be mentioned here (Perley et al., 2009, ApJ, 696, 1871; Gao et al., 2017 ApJ, 837, 50).

* Thank you for this great point. We've now included GRB 070809 with the proper citation. We now also include GRBs 050724A and 070714B in our analysis and figures, following Gao+17. Following Rossi+20 and D'Avanzo+09, we do not include 061006 due to likely host galaxy contamination in the light curve, and include the rationale for this decision in a footnote. We also now mention that kilonova claims have been made for GRB 080503 in the second paragraph of section 2.4 (~l. 320), but we do not include it because of the uncertainty in the burst's redshift.

- Please note that at line 454 061201 and 060121 are included among those with a claimed kilonova, but I could not find any reference to this finding, only strong constraints in e.g., Gompertz+18, Rossi+20.

* Thank you for pointing this out. Ascenzi+ had included 061201 as a 'possible' kilonova candidate; however, we have decided to exclude this from our list of kilonova candidates. GRB 060121 should not have been included (this was a mistake), and we have now removed it.

- l. 409-412 This is certainly the simplest approach. But both Gompertz+18, and Rossi+20 have used more sophisticated methods to obtain light curves in the rest frame of the GRB. The first interpolating the light curves of AT2017gfo, the second from SED fitting and spectroscopy. They also provide photometry from the spectroscopy that can be used in this work, which would probably benefit from the u-band light curve of AT2017gfo. The authors should also stress that this approach, although could be argued that is less precise, is not a weakness for this work, given that the aim is not to look for particular cases, but for the general properties of a big sample of kilonovae. However, the authors should provide an estimate of the systematic error that is introduced by considering the nearest band, compared to approach by Gompertz+18, and Rossi+20

* Thank you for this point. We have calculated the median percentage errors of our AT2017gfo luminosity approximations using the SEDs in Kasen et al., 2017. Specifically, we calculated the difference in luminosity of observations whose true rest-frame wavelength is at the "edge" of a band and that we get assuming the pivot band wavelength. We find median errors range from 3-37 percent. We have added a few sentences describing the result of these error calculations and their implications in the text (Section 3.1, approx. l. 380-390).

- Viewing angle:
l.636-638 
However, both Gompertz+18 and Rossi+20, conclude that the angle is not important, and the large range in luminosity is likely due to other physical properties and merger type. The authors should consider those conclusions. The authors should also check if selection effects are important, as AT 2017gfo and short GRBs have been discovered after different sources, i.e., GWs vs GRBs, with the first once only detectable at low redshifts, and the second ones detectable only if seen pole-on.

* Thanks to the referee for this point. We were motivated to re-read Gompertz+18 in which they allude to viewing angle versus ejecta properties in the last paragraph of their Section 5. The authors there conclude that the distribution of kilonova luminosities is within the range expected for various in ejecta geometry and/or ejecta properties. We do not believe that the authors there conclude that viewing angle is *not* important, more that the variation could be naturally explained by variations in ejecta properties (and we agree with these authors). We have also re-read Rossi+20. There, they do make a case that the range of luminosities cannot be explained by the viewing angle difference *alone* between GW170817 and SGRBs, but their statements are model dependent. Similar to Gompertz+18, our reading of Rossi+20 is *not* that viewing angle does not affect the overall colors/luminosities. Rather, we believe that they mean in specific cases, viewing angle is not enough to account for the discrepancy in luminosities.

What we attempt to do here is consider the effects of viewing angle on the full sample of short GRB kilonova candidates and their colors (when available). As these are all either (i) brighter in the optical than AT~2017gfo or (ii) show bluer colors than AT~2017gfo (e.g., 160821B), we think it is fair to point out that the pole-on viewing angle of short GRB kilonovae would overall bias us to observe bluer kilonovae. In reality, we believe the discrepancy in luminosities and colors is a combination of all of these factors, and it will take a few more GW-detected "off-axis" kilonovae to understand the truth. We have softened the original language to reflect this discussion in the second paragraph of Section 3.3 (approx. l. 570-590).

- comparison with Ascenzi+19 at l.1067 
This is not fair: excluding 130603B, for which there is just one detection in the K band, their fig. 5 shows Mej to be well constrained. Vej is less constrained, though. It should be noted that their method is also based 
on K17 models. Most important, their results show that no observations are consistent with masses <0.05Msun, which seems very different from the results presented here and in particular in Table 2. This is worth to be investigated here. There is of course a major difference: they work on detections, and do not consider the faint KN associated to 160821B.

* We have added in that this was done using the K17 models and have excluded their analysis of GRB 130603B, noting it was poorly constrained and mentioned that they do not consider 160821B. We now contrast our K17 results from upper limits with their results from detected candidate KN (last paragraph of Section 4.3, approx l. 830-840).

Minor comments:
##############

l.9 NIR is defined again in the main text, I think is not necessary here.

*Yes, removed.

l.26 altered?

* changed to 'modified'

l.44 often and luminous are un necessary qualitative 

*Yes, deleted both. 'Often' was intended to imply 'often observed' but this does not work. Luminous is also covered in next sentence.

l. 45 in a jet launched in a merger, -> rephrase ?

* Text has been updated

l. 46 Kouveliotou et al 1993 is not relevant here.

*Removed.

l.52-59 please select the most appropriate references, 7 lines are certainly too much for the reader. Anyway, some are perhaps well placed at the end of the paragraph (l.66-67)

*We politely decline this suggestion in the spirit of fairness to the many authors who reported independent observations and analyses of AT 2017gfo.

l.78-80 Please describe (in a sentence) why 
a NSBH merger with a BH so massive is unable 
to produce a kilonova.

*A phrase has been added to this effect, beginning l.80.

l.82 I do not understand why is important to highlight here:
"with nearly equal mass ratios".

*This was important to say in light of the previous sentence that states highly asymmetric NSBH systems will not have much, if any, EM emission.

l.126 It seems to me that Rossi+20 considers z>0.5 GRBs, too.

*Yes, this is a good point. Have updated to say the majority of previous works.

l.127 I do not think all these references are appropriate here: some works investigate single cases and apply numerical modeling and derive physical quantities for the case. Other works aimed to discern their luminosity range and derive general properties from sample, and not necessarily to discover new kilonovae (for example see the difference between Gompertz+18 and Ascenzi+19). 

*Removed Ascenzi citation.

l.133 I think Gompertz+18 do not discuss lanthanide abundances. 

*Yes, thank you. Have updated so this sentence only speaks to Ascenzi+2019.

l.158 Please be more clear: "In Section 2, we describe our ..."

*Comment incorporated in text, thank you for this point.

l.197 Ascenzi+19 is just using Gompertz+18 sample. See their Sec.2

* We've removed this line.

l.224 Y-band has capital Y.

* Capitalized Y.

l.241 About 1504024A: I see several problems here: 1) The reference to Jin is probably wrong, I suspect the right reference is ApJ 857,128 2018? But there they are using z=0.3. 2) Perhaps the most convincing argument for z~1 is given by Tanvir et al., GCN 18100, instead of Jin et al. 3) However, this makes this event extremely luminous as you also noted later in the paper. Given all this uncertainties, I ask the authors to consider this event like all other bursts with uncertain redshift and impose z=0.5. 

*Yes, this is certainly a good argument. We have changed 150424A to a burst with unknown redshift with an assumed z=0.5 and have deleted the line describing our assumption of z=1 in the text. Corresponding figures and quotes of the # bursts with unknown redshift are updated as well.

l.269-272: "which determines ..." this sentence is not necessary.

*Removed.

l.278 "point sources or known stars" just point sources

*Removed

l. 284 perhaps from sources detected within 3sigma.

*Updated in the text

l. 296-303. After checking Table 1, it seems that these constraints have been
applied to the sample in section 2.1. If so, and considering that in sec. 2.3 the authors go back on the argument of the upper limits, the text will be more clear if the constraints on the detection and upper limits are discussed just once.

* We have removed separate justification of our luminosity cut in Section 2.4 and refer to our justification in Section 2.3. Thank you for this suggestion for clarity.

l. 306. The reader would benefit from a brief description of how to get these
constraints from Fong et al., 2020. I suppose that this comes from the argument in their introduction that most of the KN events have nuLnu<5x10^41 erg/s, but it is not clear how to derive optical and NIR limits separately.

* We now report what these magnitudes correspond to in terms of peak luminosities in the text. We were somewhat more generous in accepting JHK-band limits to accommodate redder models and the poorer capabilities of ground-based NIR instruments.

l. 337 (>~21.5 mag), i.e., without m

*Removed.

l. 338 should be <10^42 erg/s in the NIR? See sec. 2.2

* We consider "low-luminosity afterglows" to have luminosities below those of AT 2017gfo, as these are most interesting for a kilonova analysis. We have clarified this in the corresponding line.

Table 1: better something like MJD or otherwise I think the date is useless, given the presence of delta_t column. The authors could fill the free space with the exposure time.

* In light of combining the "new" and "literature" samples, we have deleted the date column and replaced with an error column (not needed earlier as the majority in "new" sample were upper limits).

l.358 is delta_t<12 days in rest frame, too?

*This is in observed-frame days as unless when labeled as t_rest, times are observed. We have added a line at the end of the introduction to further clarify this point.

l.370 As kilonovae -> As both components are dominated by ...

*Updated in the text.

l.391 40.7 Mpc is the result from Cantiello et al.. Hjorth et al+17 gives 43.7. I ask to clearly refer to Cantiello only, and add a cautionary statement that Hjorth et al., found a different value with a different method. 

*Thank you for this great point - updated in the text. We have decided not to include Hjorth et al., 2017 in the text.

l.417. z=0.5 is already described above, please just refer to the appropriate section.

*Updated in the text.

Figure 2. Please highlight the known kilonovae. I warmly suggest to use red-warm colors for the NIR, and blue cold-like for the optical

* Thank you for this suggestion. Plot colors have been updated, and at least one point of each KN candidate mentioned in the text is labeled, except where labels might overlap, and KN candidate detections are labeled as stars. Multiple points of each KN candidate were not labeled because plot became too crowded.

l.434-437 I understand that 100206, 160821B are already included in Rossi et al., 2020 with similar results, please check.

* Yes, thank you for pointing out 100206. Updated in text. Rossi+20 found detections of 160821B fall below AT 2017gfo, and here in the text we focus on upper limits, so we did not include this as an already-published result. We also update these sentences to include a new analysis published in O'Connor+21 of GRB 160624A.

l.456 the reference to Jin et al-. 2019 for 070809 is necessary here. Moreover, 
I would not refer to sample papers (Gompertz, Rossi, Ascenzi) that do not discover any of those candidates.

* This is a good point. Jin et al. 2020 has been added here and in Section 2.3 where we describe kilonovae candidates in our samples. Removed Gompertz+, Ascenzi+ and Rossi+ from citations here.

l.458-461 Can elaborate more about the colors, e.g., does R differ between optical and NIR?

* A sentence has been added saying that R > 1 in optical bands is a general trend. However, broader statements about the colors of SGRB KN are not feasible as many detections are taken in a single band at a time.

l.479 This section describes several concepts that have already been introduced before, like in Sec 3.1 and in the introduction. Thus, it can be shortened.

* Thank you for this comment; repetitive information has been removed and only general sentences needed to introduce this section are included.

l. 501-507, this lines should be merged with the next paragraph, to avoid repeating and presenting twice the same models.

* These lines have been removed as they are repeated in the next paragraph.

l. 530-544 All this section is not relevant for the paper, as the mass ratio is not used further in this paper. Please remove what is not necessary to understand models and results.

* We have shortened this paragraph to one sentence, as we agree with the referee that the details are not necessary.

l. 571-587 I feel this paragraph is not relevant, too. Perhaps, just last lines important for the model of Kasen+15,+17.

* As with the above comment, we have shortened the paragraph to one sentence.

Footnote 5 should be in the main text

* Have put this into the text.

l.623-639. This is repeated in the discussion, which is a more appropriate place. 

* Agreed that this summary paragraph is repeated in the discussion, a more appropriate place. As we have decided to restructure the paper such that the discussion of the ratio analysis is included in section 3, we have created a new subsection where similar information is included, but not repeated in the discussion.

Figure 3, Bottom. Caption: the number 12 for the are different than what I find at line 627 (13 bursts).

* Thank you for seeing this mistake. It now reads '13 upper limits'.

l.689 I am not familiar with pysynphot? Can you provide a quick explanation or reference?

* We have added a few words and a citation where we mention pysynphot.

Sec 4.2 
This whole section is not well organized, although the single paragraphs are well written. For example, the AT2017gfo comparison is introduced but then discussed in the next page, together with the comparison to GRBs and models, 
which are instead introduced later. I have found this confusing. I feel everything will be more clear if, for example (just a suggestion), this changes are made: l.744-762 before 723 and l.726-743 after 790 .

* We thank the referee for this insight and accept their suggestions. For the most part, they have been implemented in the text (although given the large-scale nature of these changes, we did not bold all changes). Large rearrangements of paragraphs were made in Section 4.2 and new Section 4.3.

l.720 "In Table 2 ..." Please remove this sentence. Table 2 is introduced and better explained at lines >=744. 

* Removed sentence

l.728 please report here clearly the Mej and Vej you have obtained from Siegel+19, I can only guess that you used those at the end of page 2 of Siegel+19. Moreover, I think this long sentence should be out of the parenthesis.

* Siegel+19 parameters have been added and the citations moved out of the parenthesis. We note that we did take out the short GRB KN candidate parameters (they can be read off the figure) to reduce long paragraphs of text, in keeping with the referee's overall comment.

l.741 M19 instead of M17, typo? Moreover, I dam not sure to understand well this comment. Can you be more clear, please? Perhaps the message is that, in respect to the comparison with K17, the Mej range for AT 2017gfo is larger?

* M17 has been corrected to M19. This sentence was indeed confusing and it has been rewritten to be more clear.

l.744 How exactly the median is calculated? Is there a probability given to each Mej-Vej pair? 

* A simple median was calculated, with no probability assigned to each pair. We do not weight the median because doing so would introduce some mass or velocity prior, which we do not feel is warranted in our analysis.

l.760 Please provide an argument for the choice to concentrate on the masses and not also on the Vej.

* A justification has been modified at the beginning of the paragraph, explaining that the constraint on Vej across the range of Mej does not vary as much as Mej over the range of Vej.

Figure 4: Is Rosswog+13 in reality +14?

* Yes, thank you for pointing this out. The plot has been updated.

l.812 and Rosswog +14, too?

* Only the NSBH Rosswog+17 is cited here because all of these Mej-Vej parameters were ruled by the upper limit of 160624A. In contrast, only half of the Rosswog+14 values were ruled out. The language has been modified for clarity.

l.824 I do not understand point i) But I think this point is clear in the discussion, sec 5.2, lines 1027-1055. Please avoid quickly discussing the results, which can result ion obscure sentences, and remove line 824-832

* Thank you for this point - the lines you refer to have been removed.

l.850 these numbers are different than what I find in the caption of Figure 3

* Now that the # of bursts with limits less luminous than the NSBH model in the Figure 3 caption has been updated to 13, these numbers are in agreement.

l.986 Again, Gompertz+18 and Rossi+20 claim that the progenitor is instead more important, and tend to exclude the viewing angle.

* We have added further explanation to describe why this general trend fits with expectations. Please see earlier response to similar comment about viewing angle (in section between  major and minor comments)

l.1010 typo "kilonovae.s" -> kilonovae.

* This has been fixed, thank you.

l.1017 not clear, maybe it can vary of 1 order of magnitude?

* This line has been rewritten for clarity.

l.1100 But please see Siegel et al. (2019, Nature 569, 241). If they are correct 
more than 80 per cent of the r-process content of the Universe comes from collapsar events. Please consider this.

* This very interesting point has been added a paragraph earlier.

Section 5.3 Although very interesting, I think that only the last paragraph (l>1115) is relevant.

* Note that this is now Section 5.1, due to our restructuring. We believe that one of the most significant promises of kilonovae is their implications for contributions to the universe's r-process element budget. As an SGRB kilonova compilation paper, we feel it is important to include commentary on this subject, in light of current results. The beginning paragraphs are necessary to introduce the reader to the subject (as it has not been previously addressed in the paper), and acknowledge latest work/rate estimates. Thus, we respectfully decline the referee's suggestion and have left Section 5.3 (now Section 5.1) as is. We hope that with the significant restructuring and trimming of other sections, that this section does not read as superfluous.

l.1156-57 one of the many repetitions, it is enough to write something like "the sGRB median redshift". Please check the entire paper.

* This phrase has been shortened per the referee's suggestion. Throughout the paper, the respective citations are only put when the sample is first introduced.

l.1171-1175 I find this sentence not clear: none uncovered or only one uncovered a AT2017gfo KNa? Or 160821B is out the sample?

* This sentence has been clarified to convey that only one ground-based NIR observation had reached the luminosity of AT2017gfo at the appropriate time/band and that none had detected KN emission.

l.1233-1234 Meaning just that timescale and wavelength have been corrected for the redshift? Or the light curves have been approximated to the closest band as in section 3.2?

* The timescale has been corrected and the light curves have been approximated to the closest band as in section 3.2. This has been clarified in the text.

l.1241 Please show how much exposure time you assumed to reach such limits for 
e.g., a ground-based 8 m telescope. Moreover, given that some reader may wonder, please specific that these are 3sigma upper limits (I guess).

* Yes, thank you for this point. We have added that this is based on a 30-minute exposure with an 8 m telescope

l.1281 m=27.5 see previous comment.

* This has also been resolved in the text.

l.1318 Summarize here again how many have a measured redshift. This is the number to be compared with Gompertz+18, Rossi+20 and Ascenzi+19. Then, when providing the fraction of upper limits that probe luminosity deeper than a model (or AT 2017gfo), please provide also the numbers for only the ones with measured redshift.

* Added the number with confirmed redshift but since we do not compare our sample size to previous works here and only say our conclusions are consistent, the citations to Gompertz+18, Rossi+20 and Ascenzi+19 are left in. The first bullet point has also been updated to include percentages of bursts with known redshift.

l.1334 optical upper limits? 

* Some of these are NIR (for example, those of 160624A). Is the referee asking to specify what fraction are optical?

References:
Abbot 2020c and d are the same

* Thank you, this has been resolved.

Data editor's review:
One of our data editors has reviewed your manuscript and has the following suggestion(s) to help improve the data, software citation and/or overall content. Please treat this as you would a reviewer's comments and respond accordingly in your report to the science editor. Questions can be sent directly to the data editors at data-editors@aas.org.

It is great the authors are using \software to highlight the code used in the manuscript but citation should be given when known, e.g. astropy (The Astropy Collaboration 2013, 2018), Numpy (Harris, Millman & Oliphant 2020), and Scipy (Jones et al. 2001). In addition, it is not clear why IRAF (Tody 1986, Tody 1993), HOTPANTS (Becker 2015), Astroalign (Beroiz et al. 2020), astrometry.net (Lang et al. 2010), & gwemlightcurves (Coughlin et al. 2019, 2020) are not included.

* Thank you for this comment. We have added the proper citations in \software

==> unpublished.tex <==
\startlongtable
\tabletypesize{\footnotesize}
\savetablenum{1}
\begin{deluxetable*}{lclcCCcRc}
\centering
\tablecolumns{9}
\tabcolsep0.07in
\tablewidth{0pc}
\tablecaption{Log of New Sample of Short GRB Observations
\label{tab:unpub}}
\tablehead {
\colhead {GRB}		&
\colhead {$z$}		&
\colhead {Telescope/Instrument}	&
\colhead {Date}	&
\colhead {$\delta t$}	&
\colhead {Filter}	&
\colhead {$3\sigma$ limit}	&
\colhead {$\nu L_{\nu}$}	&
\colhead {Reference}	
\\
\colhead {}		&
\colhead {}		&
\colhead {}	&
\colhead {(UT)}	&
\colhead {(days)}	&
\colhead {}        &
\colhead {(AB mag)}	&
\colhead {(erg/s)}	&
\colhead {}		
}
\startdata
130313A &  0.5$^{\dagger}$ & Gemini-S/GMOS & 2013-03-14 & 0.62 & i & $>$25.7 & < 7.3 \times 10^{41} & 1 \\
  &  & NOT/ALFSOC & 2013-03-14 & 0.42 & i & $>$23.4 & < 6.1 \times 10^{42} & 2\\
 &  & TNG & 2013-03-14 & 0.56 & r & $>$25.0 & < 1.7 \times 10^{42} & 3 \\
130822A & 0.154 & Gemini-N/GMOS & 2013-08-13 & 0.88 & i & $>$24.5 & < 1.5 \times 10^{41} & 4 \\
& & UKIRT/WFCAM & 2013-08-28 & 5.69 & H & $>$22.8 & < 3.4 \times 10^{41} & 1 \\
& & UKIRT/WFCAM & 2013-08-29 & 6.69 & J & $>$22.0 & < 9.4 \times 10^{41} & 1 \\
130912A &  0.5$^{\dagger}$ & WHT/ACAM & 2013-09-13 & 0.84 & g & $>$24.1 & < 2.2 \times 10^{42} & 5 \\
&  & WHT/LIRIS & 2013-09-13 & 0.88 & J & $>$22.1 & < 1.3 \times 10^{43} & 1 \\
 &  & HJT/RATIR & 2013-09-13 & 1.04 & r & $>$23.3 & < 8.5 \times 10^{42} & 6 \\
 &  & HJT/RATIR & 2013-09-13 & 1.04 & i & $>$23.3 & < 6.5 \times 10^{42} & 6 \\
 &  & HJT/RATIR & 2013-09-13 & 1.04 & J & $>$22.1 & < 1.3 \times 10^{43} & 6 \\
 &  & UKIRT/WFCAM & 2013-09-13 & 1.2 & J & 22.7 $\pm$ 0.4 & < 7.4 \times 10^{42} & 1 \\
 &  & UKIRT/WFCAM & 2013-09-13 & 1.2 & H & $>$22.0 & < 1.1 \times 10^{43} & 1 \\
&  & WHT/LIRIS & 2013-09-20 & 7.71 & J & $>$22.8 & < 6.8 \times 10^{42} & 1 \\
& & Magellan/FourStar & 2013-09-24 & 11.92 & J & $>$23.7  & < 2.9 \times 10^{42} & 1 \\
140903A & 0.351 & MMT/MMTCam & 2014-09-11 & 7.53 & r &  $>$22.6  & < 6.8 \times 10^{42} & 1 \\
  &  & MMT/MMTCam & 2014-09-11 & 7.50 & i &  $>$22.9  & < 4.3 \times 10^{42} & 1 \\
141212A & 0.596 & Gemini-N/GMOS & 2014-12-13 & 0.69 & i &  $>$25.2  & < 1.8 \times 10^{42} & 1 \\
  &  & Gemini-N/GMOS & 2014-12-14 & 1.75 & i &  $>$25.2  & < 1.8 \times 10^{42} & 1 \\
150120A & 0.46 & Gemini-N/GMOS & 2015-01-20 & 0.08 & i & $>$26.0 & < 4.6 \times 10^{41}  & 1 \\
 &  & Gemini-N/GMOS & 2015-01-20 & 0.08 & r & $>$26.1 & < 5.1 \times 10^{41}  & 1 \\
  &  & Gemini-N/GMOS & 2015-01-20 & 0.13 & z & $>$25.4 & < 6.6 \times 10^{41}  & 1 \\
 &  & Gemini-N/GMOS & 2015-01-22 & 2.16 & r & $>$25.7 & < 7.4 \times 10^{41} & 1 \\
150423A & 1.394 & Magellan/IMACS & 2015-04-23 & 0.10 & i & 23.6 $\pm$ 0.1 &  6.5 \times 10^{43}  & 1 \\
  &  & WHT/ACAM & 2015-04-23 & 0.67 & g & $>$25.2 & < 2.3 \times 10^{43} & 7 \\
 &  & HJT/RATIR & 2015-04-24 & 1.06 & r & $>$24.8 & < 2.7 \times 10^{43} &  8 \\
 &  & HJT/RATIR & 2015-04-24 & 1.06 & i & $>$24.7 & < 2.2 \times 10^{43} & 8 \\
 &  & HJT/RATIR & 2015-04-24 & 1.06 & z & $>$22.0 & < 2.2 \times 10^{43} & 8 \\
150831A &  0.5$^{\dagger}$ & ESO/MPG/GROND & 2015-08-31 & 0.53 & g' & $>$24.5 & < 3.6 \times 10^{42} & 9 \\
  &  & ESO/MPG/GROND & 2015-08-31 & 0.53 & r' & $>$24.2 & < 3.6 \times 10^{42} & 9 \\
 &  & ESO/MPG/GROND & 2015-08-31 & 0.53 & i' & $>$23.8 & < 4.2 \times 10^{42}  & 9 \\
 &  & ESO/MPG/GROND & 2015-08-31 & 0.53 & z' & $>$23.6 & < 4.2 \times 10^{42} & 9 \\
 &  & ESO/MPG/GROND & 2015-08-31 & 0.53 & J & $>$21.3 & < 2.7 \times 10^{43} & 9 \\
160303A &  0.5$^{\dagger}$ & UKIRT/WFCAM & 2016-03-04 & 0.84 & J & $>$22.0 & < 1.4 \times 10^{43} & 1 \\
 &  & UKIRT/WFCAM & 2016-03-04 & 0.87 & K & $>$22.0 & < 7.7 \times 10^{42} & 1 \\
 &  & HJT/RATIR & 2016-03-03 & 0.87 & r & $>$23.7 & < 5.6 \times 10^{42} & 10 \\
 &  & HJT/RATIR & 2016-03-03 & 0.87 & i & $>$23.9 & < 4.0 \times 10^{42} &  10 \\
 &  & HJT/RATIR & 2016-03-03 & 0.87 & Z & $>$22.4 & < 1.3 \times 10^{43} &  10 \\
 &  & HJT/RATIR & 2016-03-03 & 0.87 & Y & $>$21.8 & < 2.1 \times 10^{43} &  10 \\
 &  & HJT/RATIR & 2016-03-03 & 0.87 & J & $>$21.5 & < 2.2 \times 10^{43} &  10 \\
 &  & HJT/RATIR & 2016-03-03 & 0.87 & H & $>$21.4 & < 1.8 \times 10^{43} &  10 \\
 &  & ESO/MPG/GROND & 2016-03-05 & 1.73 & i' & $>$24.3 & < 2.6 \times 10^{42} & 11 \\
 &  & ESO/MPG/GROND & 2016-03-05 & 1.73 & z' & $>$24.4 & < 2.0 \times 10^{42} & 11 \\
 &  & MMT/MMTCam & 2016-03-04 & 3.90 & r & $>$25.6 & < 9.5 \times 10^{41} & 1 \\
  &  & MMT/MMTCam & 2016-03-14 & 10.82 & i & $>$24.5 & < 2.2 \times 10^{42} & 1 \\
160408A &  0.5$^{\dagger}$ & Gemini-N/GMOS  & 2016-04-08 & 0.05 & r & 24.8 $\pm$ .1 & 2.1 \times 10^{42} & 1 \\
  &  & Gemini-N/GMOS & 2016-04-09 & 0.97 & r &  $>$25.5 & < 1.1 \times 10^{42} & 1 \\
160410A &  0.5$^{\dagger}$ & UKIRT/WFCAM & 2016-04-11 & 1.06 & J & $>$22.2 & < 1.2 \times 10^{43} & 1 \\
  &  & UKIRT/WFCAM & 2016-04-11 & 1.09 & K & $>$21.8 & < 9.4 \times 10^{42} & 1 \\
 &  & NOT/ALFSOC & 2016-04-11 & 1.68 & r &  $>$25.0 & < 1.7 \times 10^{42} & 12 \\
160411A &  0.5$^{\dagger}$ & Gemini-S/GMOS & 2016-04-11 & 0.34 & i & 23.3 $\pm$ 0.2 & 6.5 \times 10^{42} & 1 \\
 &  & ESO/MPG/GROND & 2016-06-11 & 0.34 & g' &  $>$23.6 & < 8.0 \times 10^{42} & 13 \\
 &  & ESO/MPG/GROND & 2016-06-11 & 0.34 & r' &  $>$23.8 & < 5.0 \times 10^{42} & 13 \\
 &  & ESO/MPG/GROND & 2016-06-11 & 0.34 & i' &  $>$23.1 & < 8.4 \times 10^{42} & 13 \\
 &  & ESO/MPG/GROND & 2016-06-11 & 0.34 & z' &  $>$22.9 & < 8.2 \times 10^{42} &  13 \\
 &  & ESO/MPG/GROND & 2016-06-11 & 0.34 & J &  $>$21.3 & < 2.7 \times 10^{43} & 13 \\
 &  & ESO/MPG/GROND & 2016-06-11 & 0.34 & H &  $>$20.8 & < 3.2 \times 10^{43} & 13 \\
160601A &  0.5$^{\dagger}$ & DCT/LMI & 2016-06-03 & 1.60 & r &  $>$25.0 & < 1.7 \times 10^{42} & 14 \\
160612A$^{\ddagger}$ &  0.5$^{\dagger}$ & UKIRT/WFCAM & 2016-06-15 & 2.69 & J &  $>$23.7 & < 2.9 \times 10^{42} & 1 \\
  &  & UKIRT/WFCAM & 2016-06-18 & 5.74 & J &  $>$23.1 & < 5.3 \times 10^{42} & 1 \\
160624A & 0.483 & UKIRT/WFCAM & 2016-06-25 & 1.05 & J & $>$23.4 & < 3.4 \times 10^{42} & 1 \\
  &  & Gemini-N/GMOS & 2016-06-24 & 0.05 & r & $>$24.8 & < 1.9 \times 10^{42} & 1 \\
 &  & Gemini-N/GMOS & 2016-06-24 & 0.003 & r & $>$25.5 & < 1.0 \times 10^{42} & 15 \\
  &  & $HST$/ACS & 2016-06-27 & 3.36 & F606W & $>$27.7 & < 1.3 \times 10^{41} & 1 \\
 &  & $HST$/WFC3 & 2016-06-28 & 4.27 & F125W & $>$27.5 & < 8.2 \times 10^{40} & 1 \\
 &  & $HST$/WFC3 & 2016-06-28 & 4.33 & F160W & $>$27.3 & < 7.4 \times 10^{40} & 1 \\
161001A & 0.891 & ESO/MPG/GROND & 2016-10-10 & 0.12 & J &  $>$21.3 & < 1.1 \times 10^{44} & 16 \\
170112A &  0.5$^{\dagger}$ & UKIRT/WFCAM & 2017-01-01 &  1.17 & J & $>$21.3  & < 2.8 \times 10^{43} & 1 \\
170127B &  0.5$^{\dagger}$ & UKIRT/WFCAM & 2017-01-28 & 0.55 & J &  $>$21.0 & < 3.5 \times 10^{43} & 1 \\
  &  & NOT/ALFSOC & 2017-01-27 & 0.19 & r &  $>$23.4 & < 7.7 \times 10^{42} & 17 \\
170428A  & 0.454  & MMT/MMTCam & 2017-05-01 & 3.07 & i & $>$23.7 & < 3.6 \times 10^{42} & 1 \\
 &  & MMT/MMTCam & 2017-05-02 & 4.08 & i & $>$24.4 & < 1.9 \times 10^{42} & 1 \\
 &  & UKIRT/WFCAM & 2017-05-04 & 6.24 & J &  $>$22.0 & < 1.1 \times 10^{42} & 1 \\
  &  & UKIRT/WFCAM & 2017-05-05 & 7.22 & J &  $>$22.7 & < 5.9 \times 10^{42} & 1 \\
 &  & UKIRT/WFCAM & 2017-05-06 & 8.24 & J &  $>$22.7 & < 5.9 \times 10^{42} & 1 \\
 &  & UKIRT/WFCAM & 2017-05-08 & 10.23 & J &  $>$22.5 & < 7.1 \times 10^{42} & 1 \\
170524A &  0.5$^{\dagger}$ & UKIRT/WFCAM & 2017-05-25 & 0.79 & K &  $>$21.3 & < 1.5 \times 10^{43}  & 1 \\
  &  & UKIRT/WFCAM & 2017-05-27 & 2.76 & K &  $>$21.5 & < 1.2 \times 10^{43}  & 1 \\
180715A$^{\ddagger}$ & 0.5$^{\dagger}$ & UKIRT/WFCAM & 2017-07-16 & 0.52 & J & $>$21.0 & < 3.4 \times 10^{43} & 1 \\
 &  & Gemini-S/GMOS & 2017-07-16 & 0.54 & r & $>$24.0 & < 4.3 \times 10^{42} & 1 \\
 &  & UKIRT/WFCAM & 2017-07-17 & 1.51 & J & $>$20.9 & < 4.1 \times 10^{42} & 1 \\
 &  & UKIRT/WFCAM & 2017-07-18 & 2.58 & J & $>$21.7 & < 1.8 \times 10^{43} & 1 \\
 &  & UKIRT/WFCAM & 2017-07-23 & 7.54 & J & $>$21.4 & < 2.4 \times 10^{43} & 1 \\
180718A$^{\ddagger, a}$ &  0.5$^{\dagger}$ & Gemini-N/GMOS & 2018-07-19 & 1.50 & r &  $>$25.2 & < 1.4 \times 10^{42}  & 1 \\
180727A &  0.5$^{\dagger}$ & Magellan-Clay/LDSS3 & 2018-07-29 & 1.66 & i &  $>$24.2 & < 2.9 \times 10^{42}  & 1 \\
180805B &  0.661 & Magellan-Baade/IMACS & 2018-08-06 & 0.80 & r & $>$24.2 & < 7.1 \times 10^{42} & 1 \\
  &  & ESO/HAWK-I & 2018-08-06 & 0.70 & J & $>$24.4 & < 3.0 \times 10^{42} & 18 \\
 &  & ESO/FORS2 & 2018-08-06 & 0.82 & R & $>$25.7 & < 1.8 \times 10^{42} & 18  \\
 &  & NTT/EFOSC2 & 2018-08-06 & 0.74 & i & $>$25.0 & < 2.8 \times 10^{42} & 19 \\
 &  & UKIRT/WFCAM & 2018-08-05 & 0.04 & J & $>$22.3 & < 2.1 \times 10^{43} & 1 \\
 &  & UKIRT/WFCAM & 2018-08-06 & 1.04 & J & $>$22.1 & < 2.6 \times 10^{43} & 1 \\
181126A &  0.5$^{\dagger}$ & Gemini-N/GMOS & 2018-11-26 & 0.18 & z & $>$25.3 & < 8.9 \times 10^{41} & 20 \\
  &  & Keck I/MOSFIRE & 2018-11-26 & 0.18 & K_s & $>$23.6 & < 1.8 \times 10^{42} & 21 \\
190427A$^{\ddagger}$ &  0.5$^{\dagger}$ & NOT/ALFSOC & 2019-04-27 & 0.02 & r & $>$23.5 & < 6.9 \times 10^{42} & 22 \\
191031D &  0.5$^{\dagger}$ & MMT/Binospec & 2019-11-01 & 0.18 & r & $>$24.1 & < 4.1 \times 10^{42} & 1 \\
  &  & MMT/Binospec & 2019-11-01 & 0.18 & z & $>$22.6 & < 1.1 \times 10^{43} & 1 \\
 &  & MMT/Binospec & 2019-11-02 & 1.19 & r & $>$24.4 & < 3.1 \times 10^{42} & 1 \\
 &  & HJT/RATIR & 2019-11-01 & 0.21 & r & $>$22.8 & < 1.4 \times 10^{42}  & 23 \\
 &  & HJT/RATIR & 2019-11-01 & 0.21 & i & $>$23.1 & < 8.4 \times 10^{42} & 23 \\
 &  & Gemini-N/GMOS & 2019-11-02 & 1.30 & r & $>$24.8 & < 2.0 \times 10^{42} & 24 \\
200623A$^{\ddagger,a}$ &  0.5$^{\dagger}$ & LBT/LBC & 2020-06-25 & 2.11 & r & $>$26.0 & < 6.9 \times 10^{41} & 25 \\
201221D & 1.0 & MMT/MMIRS & 2020-12-22 & 0.40 & J & $>$21.9 & < 1.5 \times 10^{43} & 1
\enddata
\tablecomments{\textbf{Data References}: (1) - This work, (2) - \cite{GCN14301}, (3) - \cite{GCN14307}, (4) - \cite{GCN15121}, (5) - \cite{GCN15224}, (6) - \cite{GCN15226}, (7) - \cite{GCN17747}, (8) - \cite{GCN17754}, (9) - \cite{GCN18219}, (10) - \cite{GCN19146}, (11) - \cite{GCN19144}, (12) - \cite{GCN19300}, (13) - \cite{GCN19292}, (14) - \cite{GCN19497} (15) - \cite{GCN19565}, (16) - \cite{GCN19975}, (17) - \cite{GCN20549}, (18) - \cite{GCN23086}, (19) - \cite{GCN23090}, (20) - \cite{GCN23458}, (21) - \cite{GCN23462}, (22) - \cite{GCN24265}, (23) - \cite{GCN26121}, (24) - \cite{GCN26147}, (25) - \cite{GCN28034} \\
\textbf{Redshift References}: This work (GRB\,180805B), %180805B
\cite{GCN15178_Wiersema}, %130822
\cite{Troja+2016}, %140903A
\cite{GCN17177}, %141212A
\cite{GCN17358}, %150120A
\cite{Selsing+2019}, %150423A
\cite{GCN19565}, %160624A 
\cite{GCN21059}, %170428A
\cite{GCN29132} %201221D
\\
$^{\dagger}$ Redshift unknown, $z=0.5$ taken as fiducial value in analysis \\
$^{\ddagger}$ \textit{Swift}-BAT detected only, entire BAT region covered by observations \\
$^{a}$ Limit applies to partial coverage of BAT localization \\}
\end{deluxetable*}
